Information Rates with Non Ideal Photon Detectors in Time-Entanglement Based QKD

We develop new methods of quantifying the impact of photon detector imperfections on achievable secret key rates in Time-Entanglement based Quantum Key Distribution (QKD). We address photon detection timing jitter, detector downtime, and photon dark counts and show how each may decrease the maximum achievable secret key rate in different ways. We begin with a standard Discrete Memoryless Channel (DMC) model to get a good bound on the mutual information lost due to the timing jitter, then introduce a novel Markov Chain (MC) based model to characterize the effect of detector downtime and show how it introduces memory to the key generation process. Finally, we propose a new method of including dark counts in the analysis that shows how dark counts can be especially detrimental when using the common Pulse Position Modulation (PPM) for key generation. Our results show that these three imperfections can significantly reduce the achievable secret key rate when using PPM for QKD. Additionally, one of our main results is providing tooling for experimentalists to predict their systems' achievable secret key rate given the detector specifications.

==> commented-out.tex <==
   \begin{comment}
    \begin{tikzpicture}
        \draw (4,0) circle[x radius=0.2cm, y radius=1cm];
        \draw (5,0) circle[x radius=0.2cm, y radius=1cm];
        \draw (4,1) --(4.5,1) node[above]{Nonlinear Crystal} -- (5,1) ;
        \draw (4,-1) -- (5,-1);
        % \draw (7, 0) node[right]{$ \ket{\phi} = \frac{1}{\sqrt{N}}\int_{t_0}^{t_0+t_f} \ket{t_A}\ket{t_B} dt$};
        \draw[ultra thick, ->, red] (0,0) node[left, black]{Pump} -- (4.5,0);
        \draw[ultra thick, -, blue] (4.5,0) -- (9,2) node[right, black]{};
        \draw[ultra thick, -, blue] (4.5,0) -- (9,-1) node[right, black]{};       
        \draw[ultra thick, -, green] (4.5,0) -- (9,1) node[right, black]{};         \draw[ultra thick, blue] (9,0.5) circle[x radius=0.4cm, y radius=1.5cm];
\draw[ultra thick, -, green] (4.5,0) -- (9,-2) node[right, black]{};                \draw[ultra thick, green] (9,-0.5) circle[x radius=0.4cm, y radius=1.5cm];
    \end{tikzpicture}
    \end{comment}
    % $ \ket{\phi} = \frac{1}{\sqrt{2}}(\ket{\textcolor{black}{S}}_A\ket{\textcolor{black}{S}}_B + \ket{\textcolor{black}{L}}_A \ket{\textcolor{black}{L}}_B)$

\begin{abstract}
%\boldmath
In modern implementations of QKD, we establish a cryptographically secure encryption key between two communicating parties by distributing entangled photons between them. In theory, security is guaranteed by the fact that any eavesdroppers attempting to measure the photons will disturb their entanglement, leading to channel errors which can be discarded in post-processing steps. These entangled photons are most commonly produced using an SPDC crystal, wherein each photon passing through has a chance of spontaneously splitting into an entangled photon pair. The simplest way to extract key bits from these photons is measuring their polarization, a method which yields us one key bit per photon at best. Unfortunately, the SPDC effect occurs fairly rarely, leading to "photon-scarce" conditions that call for alternative methods. One promising method involves using the time of arrival (ToA) of the photons at each detector to extract data. This is because it turns out that polarization isn't the only thing that's entangled; both photons in the pair are created at the same time, resulting in time-entanglement. This leads to a strong correlation between the ToAs observed at each detector, where we can  use specially-designed binning schemes to extract more than one key bit per photon. However, there is a limit to how much improvement we can squeeze out by changing our method of bit extraction -- it seems to be the case that with current hardware, QKD is not yet able to deal with the immense amounts of internet traffic supported by modern cryptographic "infrastructure". Therefore we must take the initiative to design our methods with the hardware of the future -- in which our detectors and photon sources are greatly improved -- in mind. In doing this, we realize that there are more pitfalls than one might expect. In this paper, we will explore the key rates we can achieve with this bit extraction method and introduce the pitfalls we observed and how to get around them.

\end{abstract}
